RobotCore: An Open Architecture for Hardware Acceleration in ROS 2

Hardware acceleration can revolutionize robotics, enabling new applications by speeding up robot response times while remaining power-efficient. However, the diversity of acceleration options makes it difficult for roboticists to easily deploy accelerated systems without expertise in each specific hardware platform. In this work, we address this challenge with RobotCore, an architecture to integrate hardware acceleration in the widely-used ROS 2 robotics software framework. This architecture is target-agnostic (supports edge, workstation, data center, or cloud targets) and accelerator-agnostic (supports both FPGAs and GPUs). It builds on top of the common ROS 2 build system and tools and is easily portable across different research and commercial solutions through a new firmware layer. We also leverage the Linux Tracing Toolkit next generation (LTTng) for low-overhead real-time tracing and benchmarking. To demonstrate the acceleration enabled by this architecture, we use it to deploy a ROS 2 perception computational graph on a CPU and FPGA. We employ our integrated tracing and benchmarking to analyze bottlenecks, uncovering insights that guide us to improve FPGA communication efficiency. In particular, we design an intra-FPGA ROS 2 node communication queue to enable faster data flows, and use it in conjunction with FPGA-accelerated nodes to achieve a 24.42% speedup over a CPU.

==> imgs/architecture.tex <==

\begin{figure*}[!t]
    \centering
    \scalebox{0.6}{
    \tikzset{
      state/.style={
        rectangle, rounded corners, draw=gray!80, fill=gray!20, thick,
        minimum height=2em, inner sep=10pt, text centered},
      state2/.style={
        rectangle, rounded corners, draw=black, fill=gray!70, thick,
        minimum height=2em, inner sep=10pt, text centered},
      epath/.style={draw, <->, shorten <=1pt, shorten >=1pt},
      cir/.style={draw, circle, fill, inner sep=2.5pt, text=white}
    }
    \begin{tikzpicture}[->, >=latex, line width=0.75pt]
      \draw[fill=white, color=white] (-10.8,-4.5) rectangle (9.2,4.5);
      
      %%%%%%%%%
      % titles
      %%%%%%%%%      
      %\node[text width=2.5cm] (mug) at (12.6,-4.7) {\Huge ROS 2\\ HAWG};
      \node[text width=4cm] (mug) at (-12.9,9.) {\Large \tt ROS 2 C++ stack};
      %\node[text width=3.5cm] (mug) at (-12.,9.7) {\Huge \tt ROS 2\\stack};
      %\node[text width=3.5cm] (mug) at (1.,9.7) {\Huge \tt HAWG\\stack};
      \node[text width=15cm] (mug) at (2.5,9.) {\Large \tt Our open architecture for hardware acceleration};
      
      %\node[text width=2.5cm] (pilar1) at (-5.6,-4.7) {\Large pilar I};
      %\node[text width=2.5cm] (pilar2) at (1.0,-4.7) {\Large pilar II};
      %\node[text width=2.5cm] (pilar3) at (9.0,-4.7) {\Large pilar III};
      
      \node[rotate=90] (site) at (-10.6,1) {
        \large github.com/ros-acceleration %\hspace{3ex} www.xilinx.com
      };
      
      %% vitis
      %\node[state2, text width=5cm, text height=2cm, text ragged, fill=red!30] (vitis) at (-6.4,-0.7) {
      %  \texttt{Vitis \\Unified Software\\ Platform}
      %};

    %%%%%%%%%%%
    % build system
    %%%%%%%%%%%
    % build system
    \node[state, text width=7cm, text ragged]
        (buildsystem) at (-6.4, 2.) {
            {\circled{1} build system (\texttt{ament})}\\
    };
    % ament_acceleration
    \node[state, text width=7cm, text ragged, fill=green!10]
        (amentacceleration) at (-6.4, 3.2) {
            {\circled{1} \tt ament\_acceleration}\\
    };

    % ament_vitis
    \node[state, text width=2.2cm, text height=0.6cm, text ragged, fill=green!10]
        (amentvitis) at (-8.8, 4.7) {
            {\circled{1} \tt ament\_vitis}\\
    };

    % ament_jetpack
    \node[state, text width=2.6cm, text height=0.6cm, fill=gray!5, text ragged]
        (amentrocm) at (-5.6, 4.7) {
            {\circled{1} \tt ament\_jetpack}\\
    };

    % ament_more
    \node[state, text width=0.6cm, text height=1cm, fill=gray!5]
        (amentmore) at (-3.2, 4.7) {
            {\tt ...}\\
    };
    
    %%%%%%%%%%%
    % colcon
    %%%%%%%%%%%
    \node[state, text width=4.6cm, text ragged]
        (colcon) at (0.2, 2.) {
        {\circled{2} build tools (\texttt{colcon})}\\
    };

    \node[state, text width=4.6cm, text ragged, fill=green!10]
        (colconaccel) at (0.2, 3.2) {
        {\circled{2} \tt colcon-acceleration}\\
    };
    
    % vitis
    \node[state, text width=1.7cm, text height=0.6cm, text ragged] (vitis) at (-1.1, 4.8) {
        Xilinx \\Vitis
    };

    % vitis
    \node[state, text width=1.7cm, text height=0.6cm, text ragged, fill=gray!5] (cuda) at (1.4, 4.8) {
        Nvidia\\ Jetpack
    };
        

    %%%%%%%%%%%
    % firmware
    %%%%%%%%%%%
    \node[state, text width=10cm, text ragged, fill=green!10]
    (firmware) at (8.3, 2.) {
        {\circled{3} firmware}\\
    };
    \node[state, text width=10cm, text ragged, fill=green!10]
    (accelerationfirmware) at (8.3, 3.2) {
        {\circled{3} \tt acceleration\_firmware}\\
    };
    \node[state, text width=3.5cm, text height=0.5cm, text ragged, fill=green!10]
        (accelerationfirmwarekv260) at (5.0, 4.7) {
            {\circled{3} \tt acceleration\_\\firmware\_kv260}
    };
    \node[state, text width=3.5cm, text height=0.5cm, text ragged, fill=green!10]
        (accelerationfirmwarejetson) at (9.4, 4.7) {
            {\circled{3} \tt acceleration\_\\firmware\_jetson}
    };
    \node[state, text width=1cm, text height=1cm, fill=gray!5]
        (accelerationfirmwaremore) at (12.5, 4.7) {
            {\tt ...}
    };

    %%%%%%%%%%%
    % userland
    %%%%%%%%%%%
    % drivers
    \node[state, text height=0.15cm, text width=3.3cm, text ragged, fill=green!10]
        (tracing) at (-8.2, 6.3) {
            {\circled{4} tracing}\\
    };
    \node[state, text width=2.6cm, text ragged, fill=gray!5]
        (driver) at (-4.3, 6.3) {
            {drivers}\\
    };
    \node[state, text width=4.3cm, text ragged, fill=gray!5]
        (libraries) at (0.2, 6.3) {
        {libraries}\\
    };
    \node[state, text width=10cm, text ragged, fill=gray!5]
    (cloud) at (8.3, 6.3) {
        {cloud}\\
    };
    \node[state, text width=12cm, text ragged]
        (accelerationexamples) at (-3.9, 7.5) {
            {\tt image\_pipeline}\\
    };


    %%%%%%%%%%%
    % stack
    %%%%%%%%%%%
    %% userland
    \node[state, text width=3.2cm, text height=2.2cm]
      (userland) at (-12.9, 7.) {
        {\tt userland}\\
    };
    %% tooling
    \node[state, text width=3.2cm, text height=3.2cm]
      (tooling) at (-12.9, 3.4) {
        {\tt tooling}\\
    };

    %% rclcpp
    \node[state, text width=3.2cm]
      (rcl) at (-12.9, 0.8) {
        {\tt rclcpp}\\
    };

    %% rcl
    \node[state, text width=3.2cm]
      (rcl) at (-12.9, -0.25) {
        {\tt rcl}\\
    };
    %% rmw
    \node[state, text width=3.2cm]
      (rmw) at (-12.9,-1.25) {
        {\tt rmw}\\
    };
    %% adapter
    \node[state, text width=3.2cm]
      (adapter) at (-12.9,-2.3) {
        {\tt adapter}\\
    };
    %% middleware
    \node[state, text width=3.2cm]
      (middleware) at (-12.9,-3.4) {
        {\tt middleware}\\
    };


    %%%%%%%%%%%%
    % arrows  
    %%%%%%%%%%%%
    %\draw[<-, rounded corners] (-7.15,-1.2) |- ++(-0.5,-0.7) -| (amentvitis);
    
    \path[brown, epath] (accelerationexamples) to[out=-40, in=160] node[cir, pos=0.4, scale=1.5] {a} (colcon);
    \path[brown, epath] (colcon) to[out=-60, in=180] node[cir, pos=0.4, scale=1.5] {b} (amentvitis);
    \path[brown, epath] (amentvitis) to[out=0, in=120] node[cir, pos=0.4, scale=1.5] {c} (vitis);
    %\path[brown, epath, dashed] (amentacceleration) to[out=20, in=125] node[cir, pos=0.4, scale=1.5] {c} (vitis);
    
    
    \path[brown, epath] (colcon) to[out=-40, in=120] node[cir, pos=0.4, scale=1.5] {d} (accelerationfirmwarekv260);
    %\path[brown, epath, dashed] (colcon) to[out=-30, in=-30] node[cir, pos=0.4, scale=1.5] {d} (accelerationfirmware);
    
    \path[brown!50, epath] (accelerationexamples) to[out=-10, in=120] node[cir, pos=0.4, scale=1.5] {e} (colcon);
    
    \path[brown!50, epath, dashed] (accelerationexamples) to[out=-2, in=70] node[cir, pos=0.4, scale=1.5] {\small $e_2$} (vitis);
    
    \path[brown!50, epath, dashed] (accelerationexamples) to[out=0, in=100] node[cir, pos=0.4, scale=1.5] {\small $e_1$} (accelerationfirmwarekv260);
    
    %\path[black, epath] (vitis) to[out=150, in=180](amentvitis);

    % pillars
    %\path[gray, dashed, epath] (pilar1) to[out=120, in=270](buildsystem);
    %\path[gray, dashed, epath] (pilar2) to[out=120, in=270](metabuild);
    %\path[gray, dashed, epath] (pilar3) to[out=120, in=270](firmware);

    %%%%%%%%%%%%
    % source code in-picture
    %%%%%%%%%%%%

    \node[text width=14cm] (pilar1) at (5,-0.7) {\Large \texttt{\$ colcon \hspace{0.2em} build \hspace{0.2em} ---merge-install} \circledpurple{a} \circledpurple{b} \circledpurple{c} \circledpurple{d}};
    \node[text width=14cm] (pilar1) at (5,-1.4) {\Large \texttt{\$ source \hspace{0.2em} install/setup.bash}};
    \node[text width=14cm] (pilar1) at (5,-2.8) {\Large \texttt{\$ colcon \hspace{0.2em} build \hspace{0.2em} ---merge-install \hspace{0.2em} ---mixin kv260 \\ 
        \hspace{5ex} ---install-dir \hspace{0.2em} install-kv260 \\ 
        \hspace{5ex} ---build-dir \hspace{0.2em} build-kv260} \hspace{2.2em} \circledpurplehalf{e} \circledpurplehalf{ $e_1$} \circledpurplehalf{$e_2$}};
  

    \end{tikzpicture}}
%    \caption{A ROS-centric architecture for hardware acceleration}
%    \label{fig:hawgarch}
    \caption{\small \textbf{An open architecture for hardware acceleration in ROS 2}. \protect\input{other/caption_architecture}}
    \label{fig:architecture}
\end{figure*}


==> imgs/bechmarkstreams.tex <==


\begin{figure}[!h]
\setlength\extrarowheight{2pt} % for a less-cramped "look"
%\centering
\medskip
%\includegraphics[width=0.45\textwidth]{imgs/benchmarkstreams.png}
\includegraphics[width=0.45\textwidth]{imgs/benchmarkresize_only.png}
%\includegraphics[width=0.45\textwidth]{imgs/benchmarkstreams_both.png}
\bigskip
\begin{minipage}{\columnwidth}
\scalebox{0.7}{
\begin{tabular}{ l|c|c|c|c|c}
%\hline
      & \multicolumn{2}{c|}{\small \textbf{\texttt{rectify} \& \texttt{resize}}} & \multicolumn{2}{c|}{\small \textbf{Total}} & \small \textbf{Speedup}\\
      & \small \texttt{Mean} & \small \texttt{RMS} & \small \texttt{Mean} & \small \texttt{RMS} & \\
\hline
\small CPU  & 24.36 ms & 24.50 ms & 91.48 ms & 92.05 ms &  \\
%\small FPGA\footnote{Perception tasks offloaded to the FPGA. Each \emph{Component} uses its own acceleration kernel. 250 MHz clock} & 24.46 ms & 24.66 ms & 85.80 ms & 87.87 ms & 6.22\% \\
%\small FPGA\footnote{\texttt{RectifyNode} and \texttt{ResizeNode} ROS 2 \emph{Components} integrated into \texttt{RectifyResizeNodeFPGA}, using a single acceleration kernel that offloads perception tasks. 250 MHz clock.} & 23.90 ms & 24.05 ms & 66.82 ms & 67.82 ms & 26.96\% \\
\small FPGA & 19.14~ms & 19.28~ms & 69.15 ms & 70.18 ms & 24.42\% \\

%\hline
\end{tabular}}
\end{minipage}

\caption{CPU-only implementation of case study application versus FPGA version accelerated by streamlining inter-FPGA-node communication to avoid CPU-inflicted communication overheads.
Hardware acceleration achieves a $24.42\%$ speedup, calculated from the mean of the total time.
\texttt{RectifyNodeFPGAStreamlined} and \texttt{ResizeNodeFPGAStreamlined} offload perception tasks to the FPGA and leverage an AXI4-Stream interface to create an intra-FPGA ROS 2 Node communication queue.  $250$~MHz clock. 
Mean and RMS times for FPGA rectify and resize nodes both show
%%%speedups of 21.42\% and 21.33\% speedup, respectively, compared to the CPU baseline.
$\sim 21\%$ speedup over CPU baseline.
} 
%The results presented correspond with benchmarking the perception pipeline of figure \ref{fig:usecase1} during 60 seconds with LTTng trace points enabled. The FPGA acceleration kernels use a 250 MHz clock.}

\label{fig:benchmarkstreams}    
\end{figure}

==> imgs/benchmarkacceleration.tex <==
\begin{figure}[!h]
\setlength\extrarowheight{2pt} % for a less-cramped "look"
%\centering
\medskip
%\includegraphics[width=0.45\textwidth]{imgs/benchmarkintegrated.png}
\includegraphics[width=0.45\textwidth]{imgs/benchmarkintegrated_only.png}
\bigskip
\begin{minipage}{\columnwidth}
\scalebox{0.7}{
\begin{tabular}{ l|c|c|c|c|c}
%\hline
      & \multicolumn{2}{c|}{\small \textbf{\texttt{rectify} \& \texttt{resize}}} & \multicolumn{2}{c|}{\small \textbf{Total}} & \small \textbf{Speedup}\\
      & \small \texttt{Mean} & \small \texttt{RMS} & \small \texttt{Mean} & \small \texttt{RMS} & \\
\hline
\small CPU  & 24.36 ms & 24.50 ms & 91.48 ms & 92.05 ms &  \\
%\small FPGA\footnote{Perception tasks offloaded to the FPGA. Each \emph{Component} uses its own acceleration kernel. 250 MHz clock} & 24.46 ms & 24.66 ms & 85.80 ms & 87.87 ms & 6.22\% \\
\small FPGA & 23.90 ms & 24.05 ms & 66.82 ms & 67.82 ms & 26.96\% \\

%\hline
\end{tabular}}
\end{minipage}

\caption{CPU-only implementation of case study application versus FPGA version accelerated by combining nodes to avoid CPU-inflicted communication overheads.
Hardware acceleration achieves a $26.96\%$ speedup, calculated from the mean of the total time.
\texttt{RectifyNode} and \texttt{ResizeNode} ROS 2 \emph{Components} integrated into \texttt{RectifyResizeNodeFPGA} using a single acceleration kernel that offloads perception tasks. $250$~MHz clock.
}
%The results presented correspond with benchmarking the perception pipeline of figure \ref{fig:usecase1} during 60 seconds with LTTng trace points enabled. The FPGA acceleration kernels use a 250 MHz clock.}

\label{fig:benchmarkintegrated}    
\end{figure}

==> imgs/benchmarkcpu.tex <==

\begin{figure}[!h]
\setlength\extrarowheight{2pt} % for a less-cramped "look"
%\centering
\medskip
%\includegraphics[width=1\textwidth,height=0.6\textheight]{my figure}
\includegraphics[width=0.45\textwidth]{imgs/benchmarkcpu.png}
\bigskip
\begin{minipage}{\columnwidth}
\scalebox{0.7}{
\begin{tabular}{ l|c|c|c|c|c}
%\hline
%\footnote{Calculated from the \texttt{Mean} of the Total}
%\footnote{Perception tasks offloaded to the FPGA. Each \emph{Component} uses its own acceleration kernel. 250 MHz clock}
      & \multicolumn{2}{c|}{\small \textbf{\texttt{rectify} \& \texttt{resize}}} & \multicolumn{2}{c|}{\small \textbf{Total}} & \small \textbf{Speedup} \\
      & \small \texttt{Mean} & \small \texttt{RMS} & \small \texttt{Mean} & \small \texttt{RMS} & \\
\hline
\small CPU  & 24.36 ms & 24.50 ms & 91.48 ms & 92.05 ms &  \\
\small FPGA & 24.46 ms & 24.66 ms & 85.80 ms & 87.87 ms & 6.22\% \\
%\hline
\end{tabular}}
\end{minipage}
%\label{fig:benchmarkcpu}
%\caption{\small \textbf{\texttt{CPU} and \texttt{FPGA} benchmarks}. The results presented correspond with benchmarking the perception pipeline of figure \ref{fig:usecase1} during 60 seconds with LTTng trace points enabled. The FPGA acceleration kernels use a 250 MHz clock.}

\caption{CPU-only implementation of case study application versus FPGA version offloading relevant compute tasks using the Vitis Vision Library.
Hardware acceleration achieves a $6.22\%$ speedup, calculated from the mean of the total time.
}

\label{fig:benchmarkcpufpga}    
\end{figure}

==> imgs/detailedFPGATrace.tex <==
%\begin{figure*}[!t]
\begin{figure}[!t]
    \centering
    %\includegraphics[width=1.0\textwidth]{imgs/detailedFPGATrace.png}
    \includegraphics[width=1.0\columnwidth]{imgs/detailedFPGATrace2.png}
    %\includegraphics[width=0.5\textwidth]{imgs/detailedFPGATrace2.png}
    \vspace{-15pt}
    %\caption{Detailed view into one run of the FPGA accelerated kernel using the Vitis Analyzer and showing how the overhead as the data moves from the CPU to the FPGA, consumes a substantial portion of the time which can't be traced using our current LTTng tracing approach as represents a limitation.}
    \caption{Screenshot thumbnail of single run of case study FPGA-Integrated kernel accelerator using Xilinx Vitis Analyzer.
    Data transfer overheads consume a substantial portion of runtime compared to kernel computation, confirming the communication bottleneck on the FPGA, similar to CPU.}
    \label{fig:FPGATrace}
\end{figure}
%\end{figure*}

==> imgs/instrumentation.tex <==
\begin{figure*}[!b]
    \centering
    \includegraphics[width=0.9\textwidth]{imgs/instrumentation2.png}
    \caption{Trace points across the ROS 2 abstraction layers from tracing our case study computational graph (Figure~\ref{fig:usecase1}). At the userland level, highlighted in light red are the rectify and resize computations. Highlighted in light grey are computations related to the ROS~2 message-passing system.
    }
    \label{fig:instrumentation}
\end{figure*}


==> imgs/methodology.tex <==
\begin{figure}[!t]
    \centering
    \scalebox{0.5}{
        \tikzset{
              state1/.style={fill=gray!5},
              state2/.style={fill=gray!1},
              state3/.style={fill=gray!40},
        }    
        \begin{tikzpicture}[shorten >=1pt,node distance=5cm,on grid,auto]
          \tikzstyle{every state}=[fill={rgb:black,1;white,10}]
        
            \node[state,initial, state3]   (q_1)                    {A. trace graph};
            \node[state]           (q_2)  [right of=q_1]    {B. benchmark CPU};
            \node[state]           (q_3)  [above of=q_2]    {C. hardware acceleration};
                \node[state, state2]   (q_31)  [left of=q_3]    {1. accelerate nodes};
                \node[state, state2]   (q_32)  [left of=q_31]    {2. accelerate graph};
            \node[state]           (q_4)  [above of=q_3]    {D. benchmark acceleration};
        
            \path[->]
            (q_1) edge [loop above] node {LTTng}    (   )
                  edge [bend left]  node {rebuild}    (q_2)
            (q_2) edge [bend right]  node {CPU tracing}    (q_3)
            (q_2) edge [bend left]  node {reinstrument}    (q_1)
            (q_3) edge [bend right]  node {}    (q_31)
            (q_31) edge [bend right]  node {}    (q_32)
            (q_32) edge [bend left]  node {trace dataflow}    (q_31)
            (q_31) edge [bend left]  node {trace nodes}    (q_3)
            (q_3) edge [bend left]  node {rebuild}  (q_4)
            (q_4) edge [bend left]  node {acceleration tracing}  (q_3);
        \end{tikzpicture}}
    \caption{Methodology for ROS~2 hardware acceleration, using tracing and benchmarking to improve the implementation of accelerated applications.}
    %%%\vspace{-20pt}
    \label{fig:methodology}
\end{figure}



==> imgs/usecase1.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=1.0\textwidth]{imgs/usecase1_better.png}
    \caption{\small \textbf{A ROS 2 perception computational graph built using the \texttt{image\_pipeline} package}.\\ A monocular camera with distortion is simulated using Gazebo \cite{koenig2004design} and connected to ROS through the corresponding plugins that publish to \texttt{/camera/image\_raw} and \texttt{/camera/camera\_info} topics. Nodes \texttt{/acceleration/rectify/rectify\_node\_fpga} and \texttt{/acceleration/resize/resize\_node\_fpga} subscribe to the synthetic data and compose a subgraph that aims to be hardware accelerated.}
    \label{fig:usecase1}
\end{figure*}


==> other/caption_architecture.tex <==
\small

\pgfkeys{/csteps/inner color=white}
\pgfkeys{/csteps/fill color=brown}

Our contributions are highlighted in green. The architecture include the following extensions to ROS 2: \circled{1} extensions to the build system (\texttt{ament}), \circled{2} extensions to the build tools (\texttt{colcon}), \circled{3} adds a new firmware pillar to workspaces simplifying the production and deployment of acceleration kernels and \circled{4} introduces a low-overhead real-time tracing and benchmarking approach based on the Linux Tracing Toolking next generation (LTTng \cite{desnoyers2006lttng}). A walkthrough on the interaction amongst the ROS 2 packages in the open architecture is also depicted. A first invocation to \texttt{colcon build} \Circled{a} will prepare the ROS 2 workspace for hardware acceleration and deploy files in the local overlay as illustrated by \Circled{b}, \Circled{c} and \Circled{d}. 
%
\pgfkeys{/csteps/inner color=white}
\pgfkeys{/csteps/fill color=brown!50}
%
%
After that, from the overlay, a second invocation of \texttt{colcon build} with the \texttt{--mixin <target-board>} flag \Circled{e} will cross-compile \Circled{$e_1$} and produce the accelerators \Circled{$e_2$} as needed for the target accelerator. From this point on, the \texttt{colcon\_acceleration} package helps further automate additional processes.

%A walkthrough on the interaction amongst the ROS 2 packages in the open architecture is also depicted. The process starts with \texttt{colcon build}-ing the ROS 2 workspace \Circled{a}. No special flags need to be used, only the corresponding packages must be in the \texttt{src} directory of the workspace. \texttt{colcon} will build each package for the development workstation architecture. This includes the \texttt{ament\_acceleration} and \texttt{ament\_vitis} CMake macros  \Circled{b} which will deploy a series of CMake extensions into the resulting local ROS 2 overlay workspace. These extensions connect with the local Vitis installation \Circled{c} and expose its capabilities directly to ROS 2 packages. In other words,  ROS 2 packages can leverage these macros from their \texttt{CMakeLists.txt} files and use Xilinx's hardware acceleration tooling. The \texttt{firmware} packages (e.g. \texttt{acceleration\_firmware} and \texttt{acceleration\_firmware\_kv260}) are a key component of the architecture. Moving from one accelerator solution to another should require only to select across firmware solutions \Circled{d} in the ROS overlay workspace. 

%A walkthrough on the interaction amongst the ROS 2 packages in the open architecture is also depicted. A first invocation of \texttt{colcon build} \Circled{a} will prepare the ROS 2 workspace for hardware acceleration and deploy files in the local overlay as illustrated by \Circled{b}, \Circled{c} and \Circled{d}. After that, from the overlay, a second invocation of \texttt{colcon build} with the \texttt{--mixin <target-board>} flag \Circled{e} will cross-compile \Circled{$e_1$} and produce the accelerators \Circled{$e_2$} as needed for the target accelerator. From this point on, the \texttt{colcon\_acceleration} package helps further automate additional processes.
